A Simulation Tool for tccp Programs

The Timed Concurrent Constraint Language tccp is a declarative synchronous concurrent language, particularly suitable for modelling reactive systems. In tccp, agents communicate and synchronise through a global constraint store. It supports a notion of discrete time that allows all non-blocked agents to proceed with their execution simultaneously. In this paper, we present a modular architecture for the simulation of tccp programs. The tool comprises three main components. First, a set of basic abstract instructions able to model the tccp agent behaviour, the memory model needed to manage the active agents and the state of the store during the execution. Second, the agent interpreter that executes the instructions of the current agent iteratively and calculates the new agents to be executed at the next time instant. Finally, the constraint solver components which are the modules that deal with constraints. In this paper, we describe the implementation of these components and present an example of a real system modelled in tccp.

==> eptcsdata.tex <==
\providecommand{\firstpage}{120}
\providecommand{\publicationstatus}{S. Schwarz and J. Voigtl\"ander (Eds.): 29th and 30th Workshops\\
on (Constraint) Logic Programming and 24th International\\
Workshop on Functional and (Constraint) Logic Programming\\
(WLP'15/'16/WFLP'16).\\
EPTCS 234, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.234.9}{10.4204/EPTCS.234.9}}
\pdfoutput=1


==> wgmacros-TCCP.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                         %
%   Staff only for TCCP   %
%                         %
%%%%%%%%%%%%%%%%%%%%%%%%%%%

\makeatletter
\@ifpackageloaded{MnSymbol}{}{\PackageWarning{WGmacros}%
{Please load `MnSymbol' package explicitely in preamble}
\RequirePackage{MnSymbol}}
\makeatother

\input{wgmacros-support}


% now load general staff

\input{wgmacros-general}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                               %
%   overrides of general defs   %
%                               %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\renewcommand*{\MGCsym}{\mathbb{PC}} %% most general call set

% \renewcommand*{\zseq}[2][n]{\vec{#2}}

\renewcommand*{\genrule}[2]{#1 \clauseif #2}

\renewcommand*{\paradigm}[1][]{the #1\ccp\ paradigm}
\renewcommand*{\proglang}{\tccp}
\renewcommand*{\program}{set of declarations}
\renewcommand*{\programs}{sets of declarations}
\renewcommand*{\progequiv}{declarations equivalence}%\progrule\
\renewcommand*{\progrule}{process declaration}%
% \renewcommand*{\progrules}{process declarations}
\renewcommand*{\query}[1][A]{\ifempty{#1}{P}{p}rogram}
\renewcommand*{\queries}[1][A]{\query[#1]s}
\renewcommand*{\deffun}[1][A]{process}
\renewcommand*{\deffuns}[1][A]{processes}
\renewcommand*{\expression}[1][A]{\ifempty{#1}{A}{a}gent}
\renewcommand*{\expressions}[1][A]{\ifempty{#1}{A}{a}gents}

\renewcommand*{\C}[1][]{\mathbb{M}_{#1}}
\renewcommand*{\topC}{\mathbf{M}}
\renewcommand*{\botC}{\{\ecrs\}}

% \renewcommand*{\eval}[4][\alpha]{\syntaxoper{\mathcal{A}^{#1}}{#3}{{#4}}} %% semantic evaluation
\renewcommand*{\Q}[2]{\ifempty{#2}{#1}{#2 \mathbin{.} #1}} % D.A -> \Q{A}{D}
\renewcommand*{\TpSym}{\mathC{D}}
\renewcommand*{\TrSym}{\mathC{P}} %% semantics tree in P
\renewcommand*{\evalSym}{\mathC{A}}

% In Tccp the function symbol signature does not exist, the predicates are
% the defined symbols and the constraint system signature provides the
% constructor symbols
\renewcommand*{\Fsyms}{\CSys,\Psyms}
\renewcommand*{\Csyms}{\Fbox{fix}\CSys} %% constructor symbols
\renewcommand*{\Dsyms}{\Psyms} %% defined symbols

\renewcommand*{\ProgSym}{D} %% generic program=set of decls
% Insieme degli insiemi di dichiarazioni: si usa \Progs
\renewcommand*{\ProgsSym}{\mathbb{D}} %\mathit{Progs}
\renewcommand*{\Progs}[1][\CSys]{\ProgsSym^{\Psyms}_{#1}} % \mathit{Progs}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                             %
%   Subject Specific macros   %
%                             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand*{\N}{\mathbb{N}}
\newcommand*{\R}{\mathbb{R}}
\newcommand*{\Z}{\mathbb{Z}}

\newcommand*{\D}{\prog} %% generic program Alias

\newcommand*{\CCSname}{Cylindric Constraint System}
\newcommand*{\CCSshortname}{Constraint System}
\newdefinition{CCSdef}[theorem]{\CCSname}
\newsmartprefix{CCS}{\CCSshortname}
\newsmartsprefix{CCS}{\CCSshortname s}

\newcommand*{\CylConSyst}[8]{\langle #1, \annote{$\Leftarrow$}\mathord{#2}, 
    \annote{\tiny conj}#3, #4, #5, \annote{\tiny all}#6, \mathord{#7}, #8 \rangle}
\newcommand*{\CCS}{\CylConSyst{\CSdom}{\CSord}{\CSmerge}{\CSjoin}{\CSfalse}{\CStrue}{\Var}{\CShid{}{}}}
\newcommand*{\CylConSystShort}[7]{\langle #1, \annote{$\Leftarrow$}\mathord{#2}, 
    \annote{\tiny conj}#3, #4, \annote{\tiny all}#5, \mathord{#6}, #7 \rangle}
\newcommand*{\CCSshort}{\CylConSystShort{\CSdom}{\CSord}{\CSmerge}{\CSfalse}{\CStrue}{\Var}{\CShid{}{}}}
% \newcommand*{\CCSJoin}{\CCS}

% Insieme degli agenti
\newcommand*{\Agents}[1][\CSys]{\mathbb{A}^{\Psyms}_{#1}}%\mathit{Agents}
% Insieme dei "programmi" NON SERVE

\newcommand*{\Conds}[1][\CSys]{\Lambda_{#1}}%\mathit{Agents}
\newcommand*{\ValConds}[1][\CSys]{\Delta_{#1}}%\mathit{Agents}


\newcommand*{\evalC}[3][\alpha]{\syntaxoper{\bar{\evalSym}^{#1}}{#2}{{#3}}} %compact eval
\newcommand*{\TpC}[3][\alpha]{\syntaxoper{\bar{\TpSym}^{#1}}{#2}{{#3}}}%compact Tp
\newcommand*{\FC}[2][\alpha]{\syntaxoper{\bar{\FSym}^{#1}}{#2}{}}%compact fixpoint

\newcommand*{\Conf}{\mathit{Conf}}% insieme di configurazioni
%\newcommand*{\PA}{\fbox{change to $\MGC$}}
\newcommand*{\clauseif}{\ensuremath{\mathrel{\mathord{:}\mathord{-}}}}
\newcommand*{\ra}{\rightarrow}
\newcommand*{\nra}{\not\rightarrow}
\newcommand*{\tccp}{\textit{tccp}}
\newcommand*{\ntcc}{\textit{ntcc}}
\newcommand*{\ccp}{\textit{ccp}}
\newcommand*{\cc}{\textit{cc}}
\newcommand*{\tcc}{\textit{tcc}}
\newcommand*{\hcc}{\textit{hcc}}
\newcommand*{\utcc}{\textit{utcc}}

%%OPERATORI TCCP%%

\newcommand*{\askip}{\mathord{\mathsf{skip}}}%agente skip
\newcommand*{\atell}{\parensmathoper{\mathsf{tell}}}%agente tell
%\newcommand*{\aask}{\parensmathoper{\mathsf{ask}}}%agente ask
\newcommand*{\aask}[1]{\mathop{\mathsf{ask}}\ifempty{#1}{}{(#1)\ra}}
\newcommand*{\asumask}[4][i]{\sum_{#1=1}^{#2}\aask{#3_{#1}}{#4}_{#1}}
\newcommand*{\anow}[3]{\tagnow\ifempty{#1}{} {\: #1 \tagthen #2\ifempty{#3}{}{\tagelse #3}}}
\newcommand*{\anowpar}[3]{\anow{(#1)}{#2}{#3}}
\newcommand*{\ahiding}[3][]{\mathop{\exists^{#1}{#2}} {#3}}
\newcommand*{\aparallel}[2]{#1 \parallel #2}
\newcommand*{\apcall}[2]{\mathit{#1}\ifempty{#2}{}{(\mathit{#2})}}

\newcommand*{\tagelse}{\mathrel{\mathsf{else}}}
\newcommand*{\tagnow}{\mathop{\mathsf{now}}}
\newcommand*{\tagthen}{\mathrel{\mathsf{then}}}


% \newcommand*{\ordtree}{\unlhd}
% \newcommand*{\emptytree}{\Box}

%%SEQUENZE REATTIVE%%

%\newcommand*{\R}{\mathit{R}}
%\newcommand*{\Sr}{\mathcal{S}}%dominio sequenze reattive classiche
%\newcommand*{\Rconn}{\mathbb{R}_{conn}} %insieme di sequenze reattive condizionali connesse

%%MASSIMALI

\backcompatibility{\M}{\C}
\backcompatibility{\Rm}{\C}%dominio sequenze reattive condizionali massimali
\backcompatibility{\leqM}{\leqC}
\backcompatibility{\lubM}{\lubC}%[2]{{\ifempty{#2}{\bigsqcup #1}{#1 \sqcup #2}}}
\backcompatibility{\glbM}{\glbC}%[2]{{\ifempty{#2}{\bigsqcap #1}{#1 \sqcup #2}}}
\backcompatibility{\botM}{\botC}
\backcompatibility{\topM}{\topC}
\backcompatibility{\latticeM}{\latticeC}
\backcompatibility{\cpoM}{\cpoC}

\newcommand*{\prefix}{\parensmathoper{prefix}}%op prefissi

\newcommand*{\parallelstore}[2]{\mathbin{\ifempty{#1}{\breve{\parallel}}{#1\mathrel{\breve{\parallel}} #2}}}
%parallel sequenze condizionali

%TUPLE CONDIZIONALI

\newcommand*{\seqHid}[2]{\mathop{\bar{\exists}}\nolimits_{#1} #2}
\newcommand*{\cs}[2]{ #1 \rightarrowtail #2}%\Yright\llparenthesis\rrparenthesis
\newcommand*{\csC}[3]{\cs{\cond{#1}{#2}}{#3}}
\newcommand*{\ecrs}{\epsilon} %seq. reattiva condizionale vuota

%da togliere:
% \newcommand*{\crs}[3]{\ifempty{#1}{}{#1 \Rightarrow} \pair{#2}{#3}} %tupla condizionale
% \newcommand*{\crsC}[4]{\crs{\cond{#1}{#2}}{#3}{#4}} % con condizioni esplicite
% \newcommand*{\rs}{\crs{}}
% \newcommand*{\ucoRrm}{\uco{\Rrm}{\ordRrm}}%uco sequenze massimali
% \newcommand*{\ucoRr}{\uco{\Rr}{\subseteq}}%uco sequenze
% \newcommand*{\ucoTree}{\uco{\Tree}{\ordTree}}%uco alberi


%%OPERATORI SU SEQUENZE REATTIVE%%

% \newcommand*{\seq}{\mathoper{Seq}}%costruisce la sequenza
%\newcommand*{\Conn}{\mathit{Conn}}%sequenze connesse
\newcommand*{\ed}{\boxtimes}
\newcommand*{\first}{\parensmathoper{first}}%primo store di una sequenza
\newcommand*{\last}{\parensmathoper{last}}%ultimo store di una sequenza
%\newcommand*{\inc}{\Omega} %insieme seq. inconsistenti
\newcommand*{\parallelseq}[2]{\mathbin{\ifempty{#1}{\bar{\parallel}}{#1\mathrel{\bar{\parallel}} #2}}}
%parallel sequenze condizionali
%\newcommand*{\addstore}[2]{\ifempty{#1}{\mathbin{\varoast}}{#1\mathbin{\varoast}#2}}%prop constraints operatore tran
%\newcommand*{\prop}[2]{\ifempty{#1}{\mathbin{\odot}}{#1\mathbin{\odot}}#2}%prop constraints
\newcommand*{\prop}[2]{#2\mathord{\downarrow_{#1}}}%prop constraints
%\newcommand*{\remcond}{\mathoper{RemoveConditions}}%rimuovere cond.
\newcommand*{\conscond}[2] {#1 \gg \ifempty{#1}{}{#2}}%consistenza di una condizione rispetto a uno store
\newcommand*{\nconscond}[2]{#1 \ngg \ifempty{#1}{}{#2}}%INconsistenza di una condizione rispetto a uno store
\newcommand*{\soddcond}[2] {#1 \rightModels\allowbreak \ifempty{#1}{}{#2}}%soddisfazione di una condizione rispetto a uno store
\newcommand*{\nsoddcond}[2]{#1 \nrightModels \ifempty{#1}{}{#2}}%INsoddisfazione di una condizione rispetto a uno store
\newcommand*{\stutt}[1]{\parensmathoper{\mathit{stutt}}{#1}}
%\newcommand*{\tran}[1]{\Downarrow_{#1}}  %operatore trasformazione
\newcommand*{\tran}[2]{#2\mathord{\Downarrow_{#1}}}
% \ifempty{#1}{\ifempty{#2}{\Downarrow}{\Downarrow_{#1}}}{#2\Downarrow_{#1}}}
%\newcommand*{\tranaux}[1]{\downarrow_{#1}}   %operatore trasformazione ausiliario
%\newcommand*{\uncond}{\mathbin{\otimes_{c}}}
\newcommand*{\uncond}{\mathbin{\otimes}}

%%CONSTRAINT SYSTEM%%

\newcommand*{\CSc}[1][c]{#1}
\newcommand*{\CSdom}{\mathcal{C}} %insieme di constraint
\newcommand*{\CSfalse}{\mathit{false}} %insieme di constraint
\newcommand*{\CShid}[2]{\mathop{\exists}\nolimits_{#1} #2}%exists
\newcommand*{\CSimp}{\mathrel{\vdash}}%implicazione
\newcommand*{\CSnimp}{\mathrel{\nvdash}}%implicazione
\newcommand*{\CSjoin}{\mathbin{\oplus}}%join constraints
\newcommand*{\CSbigjoin}{\bigoplus}
\newcommand*{\CSmerge}{\mathbin{\otimes}}%merge constraints
\newcommand*{\CSord}{\preceq}%contrario implicazione
\newcommand*{\CStrue}{\mathit{true}} %insieme di constraint
\newcommand*{\CSys}{\mathbf{C}} %constraint system
\newcommand*{\Var}{\mathit{Var}}%variabili

%%ABSTRACT CONSTRAINT SYSTEMS%%

\newcommand*{\ACSc}[1][c]{\hat{\CSc[{#1}]}}
\newcommand*{\ACSdom}{\hat{\CSdom}} %insieme di constraint
\newcommand*{\ACShid}[2]{\mathop{\hat\exists}\nolimits_{#1} #2}
\newcommand*{\ACSimp}{\mathrel{\hat\CSimp}}%implicazione
\newcommand*{\ACSnimp}{\mathrel{\hat\CSnimp}}%implicazione
\newcommand*{\ACSjoin}{\mathbin{\hat\CSjoin}}%merge constraints
\newcommand*{\ACSmerge}{\mathbin{\hat\CSmerge}}%merge constraints
\newcommand*{\ACSord}{\mathrel{\hat{\CSord}}}
\newcommand*{\ACSys}{\hat{\CSys}} %constraint system
\newcommand*{\ACSfalse}{\hat{\CSfalse}}
\newcommand*{\ACStrue}{\hat{\CStrue}}

\newcommand*{\ACCS}{\CylConSyst{\ACSdom}{\ACSord}{\ACSmerge}{\ACSjoin}{\ACSfalse}{\ACStrue}{\Var}{\ACShid{}{}}}
\newcommand*{\ACCSshort}{\CylConSystShort{\ACSdom}{\ACSord}{\ACSmerge}{\ACSfalse}{\ACStrue}{\Var}{\ACShid{}{}}}

\newcommand*{\ACSimppn}{\mathrel{\tilde\vdash}}%implicazione positiva e negativa
\newcommand*{\ACSnimppn}{\mathrel{\tilde\nvdash}}%implicazione positiva e negativa

\newcommand*{\AseqHid}[2]{\mathop{\tilde{\exists}}\nolimits_{#1} #2}

\newcommand*{\ACScDual}[1][a]{\check{\CSc[{#1}]}}
\newcommand*{\ACSdomDual}{\check{\CSdom}} %insieme di constraint
\newcommand*{\ACSfalseDual}{\check{\CSfalse}}
\newcommand*{\ACShidDual}[2]{\mathop{\check\exists}\nolimits_{#1} #2}
\newcommand*{\ACSimpDual}{\mathrel{\check\CSimp}}%implicazione
\newcommand*{\ACSnimpDual}{\mathrel{\check\CSnimp}}%implicazione
\newcommand*{\ACSjoinDual}{\mathbin{\check\CSjoin}}%merge constraints
\newcommand*{\ACSmergeDual}{\mathbin{\check\CSmerge}}%merge constraints
\newcommand*{\ACSordDual}{\mathrel{\check{\CSord}}}
\newcommand*{\ACStrueDual}{\check{\CStrue}}
\newcommand*{\ACSysDual}{\check{\CSys}} %constraint system

\newcommand*{\ACCSDual}{\CylConSyst{\ACSdomDual}{\ACSordDual}{\ACSmergeDual}{\ACSjoinDual}{\ACSfalseDual}{\ACStrueDual}{\Var}{\ACShidDual{}{}}}

\newcommand*{\ACSetac}{\tilde{\eta}}
\newcommand*{\ACSetam}{\check{\eta}}
\newcommand*{\ACSetapm}{\cond{\ACSetap}{\ACSetam}}
\newcommand*{\ACSetap}{\hat{\eta}}
\newcommand*{\ACSinjDual}[2]{#1 \mathbin{\check{\times}} #2}
\newcommand*{\ACSinj}[2]{#1 \mathbin{\hat{\times}} #2}


%%ABSTRACT CONDITIONAL SEQUENCE%%

%abstract sequences
\newcommand*{\latticeAM}{\lattice{\AMdom}{\leqAM}{\lubAM{}{}}{\glbAM{}{}}{\topAM}{\botAM}}
\newcommand*{\cpoAM}{\cpo{\AMdom}{\leqAM}}
\newcommand*{\leqAM}{\leqC}
\newcommand*{\AMdom}{\C^{\pm}}
\monobioperator{\glbAM}{\sqcap}{\bigsqcap}
\monobioperator{\lubAM}{\sqcup}{\bigsqcup}
\newcommand*{\botAM}{\botC}
\newcommand*{\topAM}{\topC^{\pm}}

%compact abstract sequences
\newcommand*{\latticeKAM}{\lattice{\KAMdom}{\leqKAM}{\lubKAM{}{}}{\glbKAM{}{}}{\topKAM}{\botKAM}}
\newcommand*{\cpoKAM}{\cpo{\KAMdom}{\leqKAM}}
\newcommand*{\leqKAM}{\leq}
\newcommand*{\KAMdom}{\tilde{\C}^{\pm}}
\monobioperator{\glbKAM}{\wedge}{\bigwedge}
\monobioperator{\lubKAM}{\vee}{\bigvee}
\newcommand*{\botKAM}{\botC}
\newcommand*{\topKAM}{\tilde{\topC}^{\pm}}

\newcommand*{\Acs}[3][n]{[\cs{#2}{#3}]^{#1}}
\newcommand*{\AcsC}[4][n]{[\cs{\cond{#2}{#3}}{#4}]^{#1}}
\newcommand*{\Astutt}[2][n]{[\parensmathoper{\mathit{stutt}}{#2}]^{#1}}

\newcommand*{\cond}[2]{(#1 ,\allowbreak #2)} %\,

\newcommand*{\AConds}[1][\CSys]{\tilde{\Lambda}_{#1}}%\mathit{Agents}
\newcommand*{\AValConds}[1][\CSys]{\tilde{\Delta}_{#1}}%\mathit{Agents}

%\newcommand*{\Ainc}{\Omega_{\alpha}} %insieme seq. inconsistenti
%\newcommand*{\ARr}{\Rr^{\alpha}}%dominio astratto sequenze

\newcommand*{\Aprop}[2]{\ifempty{#1}{\tilde{\downarrow}}{#2 \tilde{\downarrow}_{#1}}}%prop astratta constraints
\newcommand*{\Aparallelseq}[2]{\mathbin{\ifempty{#1}{\tilde{\parallel}}{#1 \mathrel{\tilde{\parallel}} #2}}}
\newcommand*{\Asoddcond}[2]{\mathrel{\ifempty{#1}{\mathrel{\tilde\rightModels}}{#1 \mathrel{\tilde\rightModels} #2}}}
%soddisfazione di una condizione rispetto a uno store
\newcommand*{\Ansoddcond}[2]{\ifempty{#1}{\tilde{\nrightModels}}{#1 \mathrel{\tilde{\nrightModels}} #2}}
\newcommand*{\Aconscond}[2]{\ifempty{#1}{\tilde\gg}{#1 \mathrel{\tilde{\gg}} #2}}
\newcommand*{\Anconscond}[2]{\ifempty{#1}{\tilde{\ngg}}{#1 \mathrel{\tilde{\ngg}} #2}}
\newcommand*{\Auncond}{\mathbin{\tilde{\otimes}}}

\newcommand*{\cmpt}{\parensmathoper{\kappa}}
\newcommand*{\cmptrev}{\parensmathoper{\kappa^{-1}}}

% \newcommand*{\ARrm}{\mathbb{R}_{m}^{\alpha}}%dominio sequenze astratte massimali
% \newcommand*{\ATree}{\mathbb{T}^{\alpha}}%dominio alberi astratti

%%SEMANTICS%%

%% behavior
\newcommand*{\BehaQ}[4][\mathit{ss}]{\syntaxoperEXT{#3}{\BehaSym^{\mathit{#1}}}{\Q{#3}{#4}}{#2}}
\newcommand*{\BehaFinQ}[4][\mathit{ss}]{\syntaxoperEXT{#3}{\BehaSym^{\mathit{#1}}_{F}}{\Q{#3}{#4}}{#2}}

%% concrete semantics
\newcommand*{\Aa}{\eval[]{}} % [2]{#1}{#2}sem agente
\newcommand*{\Dd}{\Tp[]} %[2]{#1}{#2}sem dich.
\newcommand*{\Pp}[2]{\ifempty{#2}{\Tr[]{#1}{}}{\Tr[]{#2}{#1}}}
\newcommand*{\Qq}[2]{\Q{#2}{#1}}
% [2]{\syntaxoper{\mathcal{P}}{\ifempty{#2}{{#1}}{\Q{#2}{#1}}}{}}%semantica sequenze reattive condizionali

%\newcommand*{\B}{\mathcal{B}}%base di un proc.
\newcommand*{\Ii}{\interpC}%dominio interpretazione di un prog.

%da spostare in un altro file??

\newcommand*{\AAa}[2]{\eval[\pm]{}{#1}{#2}}%sem agente
\newcommand*{\ADd}[2]{\Tp[\pm]{#1}{#2}}%sem dich.

\newcommand*{\interpKAM}{\interpC^{\pm}}%dominio interpretazione di un prog.

\newcommand*{\AF}{\F[\pm]}
\newcommand*{\AI}{\I[\pm]}
\newcommand*{\AS}{\Sz[\pm]}

%%ABSTRACTIONS%%

\newcommand*{\alplus}{\parensmathoper{\tau^{+}}}%alpha constraint system piu
\newcommand*{\gaplus}{\parensmathoper{\gamma^{+}}}%gamma constraint system piu

\newcommand*{\alminus}{\parensmathoper{\tau^{-}}}%alpha constraint system meno
\newcommand*{\gaminus}{\parensmathoper{\gamma^{-}}}%gamma constraint system meno

\newcommand*{\alpm}{\parensmathoper{\alpha^{\pm}}}%alpha CS sequenze
\newcommand*{\gapm}{\parensmathoper{\gamma^{\pm}}}%gamma CS sequenze

\newcommand*{\Kalpm}{\parensmathoper{\tilde{\alpha}}}%alpha sequenze
\newcommand*{\Kgapm}{ \parensmathoper{\tilde{\gamma}}}%gamma sequenze

==> wgmacros-absint.tex <==
\input{wgmacros-support}

%%%%%%%%%%%%%%%%%%%%%%%%%%
%                        %
%   DOMAINS and orders   %
%                        %
%%%%%%%%%%%%%%%%%%%%%%%%%%

% Generic Concrete Domain (for preliminaries)

\newcommand*{\CC}{\mathbb{C}}
\newcommand*{\leqCC}{\sqsubseteq} %% order on Concrete Domain
\newcommand*{\nleqCC}{\nsqsubseteq} %% negated order on Concrete Domain
\monobioperator{\lubCC}{\sqcup}{\bigsqcup}
\monobioperator{\glbCC}{\sqcap}{\bigsqcap}
\newcommand*{\botCC}{\bot} %% bottom of Concrete Domain
\newcommand*{\topCC}{\top} %% top of Concrete Domain

\newcommand*{\cpoCC}{\cpo{\CC}{\leqCC}}
\newcommand*{\latticeCC}{\lattice{\CC}{\leqCC}{\lubCC{}{}}{\glbCC{}{}}{\topCC}{\botCC}}

% Default Concrete Domain (for paper body, to be localized)

\newcommand*{\lubCbigsym}{\bigsqcup}
\newcommand*{\glbCbigsym}{\bigsqcap}
\newcommand*{\lubCsym}{\sqcup}
\newcommand*{\glbCsym}{\sqcap}

\newcommand*{\C}{\CC}
\newcommand*{\leqC}{\leqCC}
\newcommand*{\geqC}{\sqsupseteq}
\newcommand*{\nleqC}{\nleqCC}
\monobioperator{\lubC}{\lubCsym}{\lubCbigsym}
\monobioperator{\glbC}{\glbCsym}{\glbCbigsym}
\newcommand*{\botC}{\botCC}
\newcommand*{\topC}{\topCC}

\newcommand*{\cpoC}{\cpo{\C}{\leqC}}
\newcommand*{\latticeC}{\lattice{\C}{\leqC}{\lubC{}{}}{\glbC{}{}}{\topC}{\botC}}

% Generic Abstract Domain (for preliminaries)

\renewcommand*{\AA}{\mathbb{A}}
\newcommand*{\leqAA}{\leq} %% order on Abstract Domain
\newcommand*{\geqAA}{\geq} %% order on Abstract Domain
\newcommand*{\nleqAA}{\nleq} %% order on Abstract Domain
\monobioperator{\lubAA}{\vee}{\bigvee}
\monobioperator{\glbAA}{\wedge}{\bigwedge}
\newcommand*{\botAA}{\bot} %% bottom of Abstract Domain
\newcommand*{\topAA}{\top} %% top of Abstract Domain

\newcommand*{\cpoAA}{\cpo{\AA}{\leqAA}}
\newcommand*{\latticeAA}{\lattice{\AA}{\leqAA}{\lubAA{}{}}{\glbAA{}{}}{\topAA}{\botAA}}

% Default Concrete Domain (for paper body, to be localized)

\newcommand*{\lubAbigsym}{\bigvee}
\newcommand*{\glbAbigsym}{\bigwedge}
\newcommand*{\lubAsym}{\vee}
\newcommand*{\glbAsym}{\wedge}

\newcommand*{\A}{\AA}
\newcommand*{\leqA}{\leqAA}
\newcommand*{\geqA}{\geqAA}
\newcommand*{\nleqA}{\nleqAA}
\monobioperator{\lubA}{\lubAsym}{\lubAbigsym}
\monobioperator{\glbA}{\glbAsym}{\glbAbigsym}
\newcommand*{\botA}{\botAA}
\newcommand*{\topA}{\topAA}

\newcommand*{\cpoA}{\cpo{\A}{\leqA}}
\newcommand*{\latticeA}{\lattice{\A}{\leqA}{\lubA{}{}}{\glbA{}{}}{\topA}{\botA}}

\newcommand*{\al}{\parensmathoper{\alpha}}
\newcommand*{\ga}{\parensmathoper{\gamma}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                               %
%   Names of Standard Domains   %
%                               %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand*{\POS}{\ensuremath{\mathcal{POS}}}

\newcommand*{\POSpreabs}[1][]{\parensmathoper{\Gamma_{#1}}}
\newcommand*{\POSabs}{\parensmathoper{\alpha_{\Gamma}}}
\newcommand*{\POSconc}{\parensmathoper{\gamma_{\Gamma}}}
\newcommand*{\POSlub}{\lubA}
\newcommand*{\POSglb}{\glbA}
\newcommand*{\POSleq}{\leqA}
\newcommand*{\POSrestrict}[2]{{#1}|_{#2}}
\newcommand*{\POSTp}{\Tp[g]}
\newcommand*{\POSinterp}{\I[g]}
\newcommand*{\POSeval}{\eval[g]}

\newcommand*{\Iff}{\leftrightarrow}

% still to be organized

\newcommand*{\KCTerms}[1][\KVsyms]{\SigTerms{\Csyms}{\Vsyms\cup #1}} %[1][\Fsyms]{\TermsSym(#1, )} %% terms
\newcommand*{\KI}{{\I[\kappa]}}
\newcommand*{\KSz}{\Sz[\kappa]}
\newcommand*{\KTerms}[1][\KVsyms]{\Terms[{\Vsyms\cup #1}]} %[1][\Fsyms]{\TermsSym(#1, )} %% terms
\newcommand*{\KTp}{\Tp[\kappa]}
\newcommand*{\KVsyms}{\widehat{\Vsyms}}
\newcommand*{\Kcut}[2][k]{#2 \lightning_{#1}}
\newcommand*{\Keval}{\eval[\kappa]}
\newcommand*{\depthk}[1][k]{\ensuremath{\mathit{depth}(#1)}}


==> wgmacros-general.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                         %
%   General definitions   %
%                         %
%%%%%%%%%%%%%%%%%%%%%%%%%%%

\input{wgmacros-absint}
\input{wgmacros-math}
\input{wgmacros-misc}
\input{wgmacros-semantics}


==> wgmacros-math.tex <==
\newcommand*{\dfn}{\coloneq}
\newcommand*{\revdfn}{\eqqcolon}

\makeatletter
\@ifpackagelater{mathtools}{2011/02/12}{%
\DeclarePairedDelimiterX{\set}[2]{\{}{\}}{#1\ifempty{#2}{}{\,\delimsize\vert\, #2}}
\DeclarePairedDelimiterX{\mset}[2]{\langle}{\rangle}{#1\ifempty{#2}{}{\,\delimsize\vert\, #2}}
}{%
\PackageWarning{WGmacros}{The version of `mathtools' package is too old, expect wrong output}
\DeclarePairedDelimiter{\set}{\{}{|}
\DeclarePairedDelimiter{\mset}{\langle}{|}
}
\makeatother

\providecommand{\annote}[1]{}

\newcommand*{\cpo}[2]{{(#1, \, \mathord{#2})}}

\newcommand*{\lattice}[6]{{(#1, \, \mathord{#2}, \,
\annote{$\vee$}\mathord{#3}, \, \mathord{#4}, \,
\annote{$\top$}\mathord{#5}, \, \mathord{#6})}}

\newcommand*{\zseq}[2][]{\overrightarrow{{#2}_{#1}}} %% indexed (short) sequence
\newcommand*{\seq}[2][n]{#2_{1}, \dots, #2_{#1}} %% indexed sequence
\newcommand*{\hoseq}[3][n]{#2{{#3}_{1}}, \dots, #2{{#3}_{#1}}}

\newcommand*{\glb}{\ensuremath{\mathit{glb}}}
\newcommand*{\lub}{\ensuremath{\mathit{lub}}}

\newcommand*{\quotient}[2]{{#1}\big/_{\! #2}}
\newcommand*{\eqClass}[2]{[{#1}]_{#2}}

\newcommand*{\PowerSet}[1]{\mathop{\powerset}(#1)}
\newcommand*{\FinPowerSet}[1]{\mathop{\powerset_{f}}(#1)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                 %
%   Macros that some package may already provide  %
%                                                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\providecommand*{\mathoper}[1]{\mathop{\mathit{#1}}\nolimits}

\providecommand*{\pair}[2]{{\langle #1, \, #2 \rangle}}
\providecommand*{\triple}[3]{{\langle #1, \, #2, \, #3 \rangle}}
\providecommand*{\quadruple}[4]{{\langle #1, \, #2, \, #3, \, #4 \rangle}}

\providecommand*{\true}{\mathit{true}}       %% simbolo di costante logica (T)
\providecommand*{\false}{\mathit{false}}     %% simbolo di costante logica (F)
\providecommand*{\id}[1][]{\mathit{id}_{#1}} %% funzione identica

\providecommand*{\True}{\mathit{True}}
\providecommand*{\False}{\mathit{False}}

\providecommand*{\nimplies}{\nRightarrow}
\renewcommand*{\implies}{\Rightarrow}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                 %
%   Symbols that some package like MnSymbol may already provide   %
%                                                                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\ProvideWarnCommand{\powerset}{\wp} 
\ProvideWarnCommand{\llbracket}{[\![}
\ProvideWarnCommand{\rrbracket}{]\!]}

\ProvideWarnCommand{\coloneqq}{\mathrel{\vcentcolon=}} %% :=
\ProvideWarnCommand{\coloneq}{\mathrel{\coloneqq}} 
\ProvideWarnCommand{\eqqcolon}{\mathrel{=\vcentcolon}} % =:

% Negated symbols
\ProvideWarnCommand{\ngg}{\not\gg} 
\ProvideWarnCommand{\nin}{\notin}
\ProvideWarnCommand{\notin}{\not\in}
\ProvideWarnCommand{\npreccurlyeq}{\not\preccurlyeq}
\ProvideWarnCommand{\nsimeq}{\not\simeq}
\ProvideWarnCommand{\nsqsubseteq}{\not\sqsubseteq}
\ProvideWarnCommand{\nrightarrowtriangle}{\not\rightarrowtriangle}
\ProvideWarnCommand{\nRightarrow}{\not\Rightarrow} 


==> wgmacros-misc.tex <==
\makeatletter
\@ifpackageloaded{listings}{
    \newcommand*{\mlst}[1]{\mbox{\lstinline[multicols=]`#1`}}
}{
    \newcommand*{\mlst}[1]{\fbox{\fbox{load package listings}\texttt{\string#1}}}
}

\@ifpackageloaded{datetime2}{
    \newcommand*{\currenttime}{\DTMcurrenttime}
}{
}
\makeatother

\providecommand*{\currenttime}{\fbox{NO TIME package}}
\providecommand*{\mathscr}{\PackageWarning{WGmacros}{no mathscr font}\mathcal} 
\providecommand*{\mathfrak}{\PackageWarning{WGmacros}{no mathfrak font}\mathcal} 

\providecommand*{\eg}   {e.g.} 
\providecommand*{\etc}  {\emph{etc}.}
\providecommand*{\ie}   {i.e.,} 
\providecommand*{\resp} {respectively}
\providecommand*{\st}   {s.t.}
\providecommand*{\wrt}  {w.r.t.}
\providecommand*{\wlg}  {w.l.o.g.}
% \providecommand*{\Wlog} {\wlg}
% 
\newcommand*{\paradigm}[1][] {\Fbox{default #1 paradigm}}
\newcommand*{\proglang}{\Fbox{default programming language}}
\newcommand*{\program}[1][A]{\ifempty{#1}{P}{p}rogram}
\newcommand*{\programs}[1][A]{\program[#1]s}
\newcommand*{\progequiv}{\program\ equivalence}
\newcommand*{\progequivs}{\progequiv s}
\newcommand*{\progrule}{\program\ rule}
\newcommand*{\progrules}{\progrule s}
\newcommand*{\query}[1][A]{\ifempty{#1}{Q}{q}uery}
\newcommand*{\queries}[1][A]{\ifempty{#1}{Q}{q}ueries}
\newcommand*{\expression}[1][A]{\ifempty{#1}{E}{e}xpression}
\newcommand*{\expressions}[1][A]{\expression[#1]s}
\newcommand*{\deffun}[1][A]{\ifempty{#1}{defined }{}function}
\newcommand*{\deffuns}[1][A]{\deffun[#1]s}


\providecommand*{\bibURLext}[2]{\draft{CONSIDER convert bib entry with `url' field!}Available at URL: \href{#1}{\texttt{#2}}}
\providecommand*{\bibURL}[1]{\draft{CONSIDER convert bib entry with `url' field!}Available at URL: \href{#1}{\texttt{#1}}}
\providecommand*{\href}[2]{\wgmWarn{\href}\underline{#2}}

\providecommand*{\email}[1]{\texttt{#1}}

\newcommand*{\xcite}[1]{[{#1}]}

%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\RequirePackage{color}

\newcommand*{\Fbox}{\fcolorbox{black}{yellow}}
\newcommand*{\Flbox}{\fcolorbox{black}{lightyellow}}
\newcommand*{\Dbox}[1]{\draft{\Fbox{#1}}}

\definecolor{aliciacolor}{RGB}{0,125,0}

\newcommand{\Ago}[2][]{\hole{\colorbox{yellow}{Santi} #1 \quad #2}}
\newcommand{\Marco}[2][]{{\color{blue}\hole{\colorbox{yellow}{Marco} #1 \quad #2}}}
\newcommand{\MarcoPN}[2]{\begin{draftpleasenote}[Marco: #1]\color{blue} #2\end{draftpleasenote}}
\newcommand{\Maria}[2][]{\hole{\colorbox{yellow}{Maria} #1 \quad #2}}
\newcommand{\Moreno}[2][]{\hole{\colorbox{yellow}{Moreno} #1 \quad #2}}

\newcommand{\Alicia}[2][]{\hole{\textbf{#1}\hfill{\color{aliciacolor}\textbf{Alicia}}\\[-1.7ex]\rule{\linewidth}{0.5mm}\\ #2}}
\newcommand{\Giovanni}[2][]{\hole{\textbf{#1}\hfill{\color{blue}\textbf{Giovanni}}\\[-1.7ex]\rule{\linewidth}{0.5mm}\\ #2}}

% nonstandard color names

\RequirePackage{xcolor}

\newcommand{\FromTo}[2]{\csname#1\endcsname[\colorbox{pink}{@#2}]}

\newcommand{\Laura}[2][]{\hole{\textbf{#1}\hfill{\color{violet}\textbf{Laura}}\\[-1.7ex]\rule{\linewidth}{0.5mm}\\ #2}}
\newcommand{\Luca}[2][]{\hole{\textbf{#1}\hfill{\color{orange}\textbf{Luca}}\\[-1.7ex]\rule{\linewidth}{0.5mm}\\ #2}}
\newcommand{\MarcoA}[2][]{\hole{\textbf{#1}\hfill{\color{orange}\textbf{MarcoA}}\\[-1.7ex]\rule{\linewidth}{0.5mm}\\ #2}}

% \newcommand{\AtAlicia}{\FromTo{Marco}{Alicia}}%[1]\Marco[\colorbox{pink}{@Alicia}]{#1}}
% \newcommand{\AtGiovanni}{\FromTo{Marco}{Giovanni}}%[1]{\Marco[\colorbox{pink}{@Giovanni}]{#1}}
% \newcommand{\AtLaura}{\FromTo{Marco}{Laura}}%[1]{\Marco[\colorbox{pink}{@Laura}]{#1}}
% \newcommand{\AtLuca}{\FromTo{Marco}{Luca}}%[1]{\Marco[\colorbox{pink}{@Luca}]{#1}}



==> wgmacros-semantics.tex <==
\makeatletter
\providecommand{\ifempty}[3]{\def\@@@temp{#1}\ifx\@@@temp\@empty#2\else#3\fi}
\@ifpackageloaded{mathtools}{}{\PackageWarning{WGmacros}%
{Please load `mathtools' package explicitely in preamble}
\RequirePackage{mathtools}}
\makeatother

\input{wgmacros-support}

%%%%%%%%%%%%%%%%%%%%%%%%%%
%                        %
%   DOMAINS and orders   %
%                        %
%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand*{\interpC}[1][]{\mathbb{I}_{#1}} %% interpretations
\newcommand*{\interpA}[1][\A]{\mathbb{I}_{#1}} %% interpretations
\newcommand*{\leqIc}{\leqC} %% order on interpretetions
\newcommand*{\leqIa}{\leqA} %% order on interpretetions
\newcommand*{\nleqIc}{\nleqC} %% order on interpretetions
\newcommand*{\nleqIa}{\nleqA} %% order on interpretetions

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                       %
%   TERMS (signature, positions, ...)   %
%                                       %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% private (just for redefinition)
\newcommand*{\mathT}{\mathcal}
\newcommand*{\TermsSym}{\mathT{T}}
\newcommand*{\LinTermsSym}{\mathT{L}{\scriptstyle\TermsSym}}
\newcommand*{\twoParsDenot}[3]{\mathop{#1}(#2, #3)}
% public

\newcommand*{\SigTerms}[2]{\twoParsDenot{\TermsSym}{#1}{#2}}
\newcommand*{\LinSigTerms}[2]{\twoParsDenot{\LinTermsSym}{#1}{#2}}

\newcommand*{\Psyms}{\Pi}       %% predicate symbols (signature)
\newcommand*{\Fsyms}{\Sigma}    %% function symbols (signature)
\newcommand*{\Csyms}{\mathT{C}} %% constructor symbols
\newcommand*{\Dsyms}{\mathT{D}} %% defined symbols
\newcommand*{\Vsyms}{\mathT{V}} %% variable symbols
\backcompatibility{\Fsym}{\Fsyms}
\backcompatibility{\Csym}{\Csyms}
\backcompatibility{\Dsym}{\Dsyms}
\backcompatibility{\Vsym}{\Vsyms}




%% terms
\newcommand*{\Terms}[1][\Vsyms]{\SigTerms{\Fsyms}{#1}}
%% constructor terms
\newcommand*{\CTerms}[1][\Vsyms]{\SigTerms{\Csyms}{#1}}

%% Linear terms
\newcommand*{\LinTerms}[1][\Vsyms]{\LinSigTerms{\Fsyms}{#1}}
%% Linear constructor terms
\newcommand*{\LinCTerms}[1][\Vsyms]{\LinSigTerms{\Csyms}{#1}} 

\newcommand*{\leqT}{\preceq} %% order on terms

% \newcommand*{\leqP}{\fbox{change}\preceq} %% order on positions
% \newcommand*{\pos}[2][]{\mathcal{O}_{#1}(#2)} %% term positions set 
\newcommand*{\append}{\cdot} %% append
\newcommand*{\replace}[3]{#1[#2]_{#3}} %% term replacement
\newcommand*{\rootPos}{\Lambda} %% root position
\newcommand*{\subterm}[2]{#1|_{#2}} %% subterm

\newcommand*{\vars}[1]{\parensmathoper{var}{#1}} %% term variables
\newcommand*{\fresh}{\ll} %% fresh variant

\newcommand*{\termres}[2]{{#1} \ifempty{#2}{}{\triangleright {#2}}}

\newcommand*{\call}[3]{\termres{\mathit{#1}\ifempty{#2}{}{\mathit{(#2)}}}{#3}}
\newcommand*{\mgc}[4][]{\call{#2}{\mbox{$\zseq[#1]{#3}$}}{#4}}

%% program (rewrite) rule
\newcommand*{\genrule}[2]{#1 \rightarrow #2}
\newcommand*{\prule}[3]{\genrule{\mathit{#1}\ifempty{#2}{}{\mathit{(#2)}}}{#3}}

\newcommand*{\mghead}[3][]{\mathit{#2}\ifempty{#3}{}{(\zseq[#1]{\mathit{#3}})}}
\newcommand*{\mgrule}[4][]{\genrule{\mghead[#1]{#2}{#3}}{#4}}

% \newcommand*{\letop}[2]{\mathop{\mathit{let}} #1 \mathrel{\mathit{in}} #2 } %% let constr. (abstract syntax)

%%%%%%%%%%%%%%%%%%%%%
%                   %
%   SUBSTITUTIONS   %
%                   %
%%%%%%%%%%%%%%%%%%%%%

\newcommand*{\Substs}{\mathit{Substs}}
\newcommand*{\CSubsts}{\Csyms\Substs} %% constructor substitutions
\newcommand*{\MGCsym}{\mathbb{MGC}}
\newcommand*{\MGC}[1][]{\MGCsym_{#1}} %% most general call set

\newcommand*{\leqS}{\preceq} %% order on substitutions
\newcommand*{\gtS}{\succ}    %% order on substitutions
\newcommand*{\eqS}{\simeq}    %% order on substitutions
\newcommand*{\neqS}{\nsimeq}    %% order on substitutions
% \newcommand*{\lubS}{\mathbin{\uparrow}} % oppure mathrel?
\monobioperator{\lubS}{\mathbin{\uparrow}}{\mathbin{\uparrow}}

\newcommand*{\emptysubst}{\varepsilon} %% empty substitution
\newcommand*{\dom}{\parensmathoper{dom}} %% domain
\newcommand*{\range}{\parensmathoper{range}} %% range
\newcommand*{\img}{\parensmathoper{img}}
\backcompatibility{\domrestriction}{\restrict}
\newcommand*{\restrict}[2]{{#1}\mathord{\restriction}_{#2}} %% domain restriction
\newcommand*{\restrictVars}[2]{\restrict{#1}{\vars{#2}}}

%%%%%%%%%%%%%%%%
%              %
%   PROGRAMS   %
%              %
%%%%%%%%%%%%%%%%

\newcommand*{\ProgsSym}{\mathbb{P}}
\newcommand*{\Progs}[1][\Fsyms]{\ProgsSym_{#1}} % \mathit{Progs}

\newcommand*{\ProgSym}{P}
\newcommand*{\prog}[1][]{\ensuremath{\ProgSym_{\mathit{#1}}^{}}} %% generic program
\renewcommand*{\P}{\prog} %% generic program Alias

\newcommand*{\CAnsw}[2]{{#1 \cdot #2}}%\talloblong\mathrel{}
\backcompatibility{\cansw}{\CAnsw}
\newcommand*{\CAleq}{\preceq}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                             %
%   REWRITING AND NARROWING   %
%                             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \RequirePackage{theorems}
\providecommand*{\starred}[2][*] {\wgmWarn{\starred}\mathrel{\mathord{#2}{}^{#1}}}


\newcommand*{\rewriteStep}[2][\genrule{l}{r}]{\xrightarrow[{#1}]{#2}}
% \newcommand*{\rewriteStep}[2][\genrule{l}{r}]{\xrightarrow[{\scriptscriptstyle #1}]{\scriptscriptstyle #2}}
\newcommand*{\rewrites}[1][]{\rewriteStep[{#1}]{}}
\newcommand*{\rewritesTo}[1][]{\starred{\rewrites[{#1}]}}
\newcommand*{\nrewrites}{\nrightarrow}
\newcommand*{\nrewritesTo}{\starred{\nrewrites}}


\newcommand*{\narrows}[2][]{\mathrel{\mathop{\leadsto}\limits^{\scriptscriptstyle #2}_{\scriptscriptstyle #1}}}
\newcommand*{\narrowsTo}[2][]{\starred{\narrows[#1]{#2}}}
\newcommand*{\narrowStep}[3][\genrule{l}{r}]{\narrows[{#1}]{\extraArg{#2}{#3}}}
\newcommand*{\nnarrows}{\not\leadsto}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                        %
%   SEMANTICS INTERPRETATION FUNCTIONS   %
%                                        %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% private (just for redefinition)
\newcommand*{\mathC}{\mathcal}
\newcommand*{\BehaSym}{\mathC{B}}
\newcommand*{\SemSym}{\mathC{S}}
\newcommand*{\TrSym}{\mathC{N}}
\newcommand*{\OsemSym}{\mathC{O}}
\newcommand*{\FSym}{\mathC{F}}
\newcommand*{\TpSym}{\mathC{P}}
\newcommand*{\evalSym}{\mathC{E}}
% public

\newcommand*{\Q}[2]{#1 \mathbin{\scriptstyle\mathit{in}} #2} % _ in _
\newcommand*{\Beha}[2][ss]{\syntaxoper{\BehaSym^{\mathit{#1}}}{#2}{}} %% general behavior macro
\newcommand*{\Sem}[2][\alpha]{\syntaxoper{\SemSym^{#1}}{#2}{}} % a semantics S
\newcommand*{\Tr}[3][]{\syntaxoperEXT{#2}{\TrSym_{#1}}{\Q{#2}{#3}}{}} %% semantics tree in P
% \newcommand*{\CA}[1]{\syntaxoper{\mathcal{CA}}{#1}{}} %% computed answers
% \newcommand*{\CAin}[2]{\CA{\Q{#1}{#2}}} %% computed answers in P

\newcommand*{\Osem}[1]{\syntaxoper{\OsemSym}{#1}{}} %% oper lfp characterization
\newcommand*{\F}[2][\alpha]{\syntaxoper{\FSym^{#1}}{#2}{}} %% general lfp macro
\newcommand*{\Tp}[3][\alpha]{\syntaxoper{\TpSym^{#1}}{#2}{{#3}}} %% general fixed-point op macro
\newcommand*{\TpN}[3][\alpha]{\iter{\Tp[{#1}]{#2}{}}{#3}} %% n-th iteration of the lfp conctruction
\newcommand*{\eval}[4][\alpha]{\syntaxoperEXT{#3}{\evalSym^{#1}}{\termres{#3}{#2}}{#4}}
\newcommand*{\evalrules}[3][\alpha]{\syntaxoper{\xi^{#1}}{#2}{#3}}
\newcommand*{\FUNeq}{\cong} %% variance on tree

\newcommand*{\I}[1][\alpha]{\Isym{#1}} %% generic interpretation
\newcommand*{\Sz}[1][\alpha]{\Ssym{#1}} %% generic specification
\newcommand*{\Rz}[1][\alpha]{\Rsym{#1}}
\newcommand*{\Isym}[1]{\mathC{I}^{#1}}
\newcommand*{\Ssym}[1]{\mathC{S}^{#1}}
\newcommand*{\Rsym}[1]{\mathC{X}^{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                          %
%   PROGRAM EQUIVALENCES   %
%                          %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand*{\ProgEquiv}[3][]{#2 \thickapprox_{#1} #3} % program equivalence
\newcommand*{\nProgEquiv}[3][]{#2 \not\thickapprox_{#1} #3} % negated program equivalence
\newcommand*{\BehaEq}[1][ss]{\ProgEquiv[\mathit{#1}]}
\newcommand*{\SemEq}[1][{\F[]{}}]{\ProgEquiv[{#1}]} %% program small-step operational equivalence


%%%%%%%%%%%%%%%%%%%
%                 %
%   PROOF TREES   %
%                 %
%%%%%%%%%%%%%%%%%%%

\newcommand{\ands}{\fbox{this should not be used, is just to prevent 
    unobserved redefinition of command \string\ands}}
\newcommand*{\sequent}[4][]{\gdef\and{\quad\hfill}
    \gdef\ands{\;\hfill\ldots\hfill\;}\global\setlabel{#1}
    {#1}\frac{\:\:#2\:\:}{\;#3\;}\;\text{\small%
\begin{tabular}{@{}l@{}} #4 \end{tabular}}}
    
\newcommand*{\twsequent}[3][]{\Fbox{OBSOLETE}\sequent[{#1}]{#2 \and #3}}

\newcommand*{\thsequent}[4][]{\Fbox{OBSOLETE}\sequent[{#1}]{#2 \and #3 \and #4}}

\newcommand*{\manysequent}[3][]{\Fbox{OBSOLETE}\sequent[{#1}]{#2 \ands #3}}

%%%%%%%%%%%%%
%           %
%   TREES   %
%           %
%%%%%%%%%%%%%

\DeclarePairedDelimiter{\Theight}{|}{|}
\newcommand*{\Tnode}[2]{\CAnsw{#1}{#2}} %% node constructor
\newcommand*{\Tpaths}{\parensmathoper{paths}}
\newcommand*{\Tmaxpaths}{\parensmathoper{maxpaths}}
\newcommand*{\Troot}{\parensmathoper{rt}} %% root node of a tree
\newcommand*{\Tsiblings}{\parensmathoper{siblings}}
\newcommand*{\Tsons}{\parensmathoper{sons}}
\newcommand*{\Tsteps}{\parensmathoper{steps}} %% steps set of a tree
\newcommand*{\Tstep}[4]{\quadruple{#1}{#2}{#3}{#4}} %% a relaxed-step in a tree
\newcommand*{\Tsubterm}[2]{\left. #1 \right\Downarrow_{#2}} %% induced subterm tree
% \newcommand*{\Tleaf}{\parensmathoper{leaf}} %% leaf nodes of a tree
\newcommand*{\Tleaves}{\parensmathoper{leaves}} %% leaf nodes of a tree

%%%%%%%%%%%%%%%%%%%%%
%                   %
%   Miscellaneous   %
%                   %
%%%%%%%%%%%%%%%%%%%%%

\newcommand*{\mgu}{\parensmathoper{mgu}} %% most general unifier

\newcommand*{\lfp}[1][]{\lfpof[{#1}]{}}
\newcommand*{\gfp}[1][]{\gfpof[{#1}]{}}
\newcommand*{\lfpof}[2][]{\mathoper{lfp}_{#1}\Braces{#2}}
\newcommand*{\gfpof}[2][]{\mathoper{gfp}_{#1}\Braces{#2}}

\newcommand*{\downiter}[2]{#1 \mathord{\downarrow} #2} %% iteration macro
\newcommand*{\iter}[2]{#1 \mathord{\uparrow} #2} %% iteration macro
\newcommand*{\sameof}[3]{#1 \mapsto \iter{#2}{#3} (\mathit{#1})}


\newcommand*{\len}{\parensmathoper{length}}
\newcommand*{\prefixtree}{\parensmathoper{prfxtree}}


% COMPATIBILITY

% \newcommand*{\restriction}{\upharpoonright}

\backcompatibility{\equivClass}{\quotient}
\backcompatibility{\rewrule}{\genrule}
\newcommand*{\rew}[2][noOpt]{\Fbox{USE \texttt{\string\rewrites}}\Fbox{$#1$}\rewrites[{#2}]}
\newcommand*{\rews}[2][noOpt]{\Fbox{USE \texttt{\string\rewritesTo}}\Fbox{$#1$}\rewritesTo[{#2}]}
\backcompatibility{\nrew}{\nrewrites}

\backcompatibility{\Subst}{\Substs}
\backcompatibility{\CSubst}{\CSubsts}
\backcompatibility{\Symbols}{\Fsyms}
\backcompatibility{\emptypos}{\rootPos}

%backward compatibility
\backcompatibility{\interp}{\interpC}
\backcompatibility{\leqI}{\leqIc}
\backcompatibility{\nleqI}{\nleqIc}


==> wgmacros-support.tex <==
% internals 

\providecommand*{\wgmWarn}[1]{\typeout{*** using WgMacros def of \string#1}}
\providecommand*{\ProvideWarnCommand}[2]{\providecommand*{#1}{\wgmWarn{#1}#2}}

\providecommand*{\backcompatibility}[2]{
  \newcommand*{#1}{\Fbox{USE \texttt{\string#2}}#2}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                      %
%   Support (General Purpose) Macros   %
%                                      %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\providecommand*{\parensmathoper}[2]{\ensuremath{\mathoper{#1}\ifempty{#2}{}{(#2)}}}
\providecommand*{\parensmathoperEXT}[3]{\ensuremath{\mathoper{#1}\ifempty{#2}{}{(#3)}}}
\providecommand*{\syntaxoper}[3]{\mathoper{#1}\BBrackets[#3]{#2}}
\providecommand*{\syntaxoperEXT}[4]{\mathoper{#2}\ifempty{#1}{}{\llbracket#3\rrbracket_{#4}}}%

\providecommand*{\BBrackets}[2][]{\ifempty{#2}{}{\llbracket#2\rrbracket_{#1}}}
\providecommand*{\Braces}[2][]{\ifempty{#2}{}{( #2 )_{#1}}}%\big\big
\providecommand*{\extraArg}[2]{\ifempty{#1}{#2}{\ifempty{#2}{#1}{#1 ,\, #2}}}
\providecommand*{\extraArgSc}[2]{\ifempty{#2}{#1}{\ifempty{#1}{#2}{#1 ;\, #2}}}

\providecommand*{\monobioperator}[3]{
  \newcommand*{#1}[2]{{\ifempty{##2}{#3##1}{##1#2##2}}}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                            %
%   Support Macros defined by theorems.sty   %
%                                            %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\providecommand*{\newsmartprefix}[2]{\wgmWarn{\newsmartprefix}}
\providecommand*{\newsmartsprefix}[2]{\wgmWarn{\newsmartsprefix}}
\providecommand*{\newdefinition}[1]{\wgmWarn{\newdefinition}\newdefinitionaux}
\providecommand*{\newdefinitionaux}[2][]{}
